Towards the Science of Security and Privacy in Machine Learning

Advances in machine learning (ML) in recent years have enabled a dizzying array of applications such as data analytics, autonomous systems, and security diagnostics. ML is now pervasive---new systems and models are being deployed in every domain imaginable, leading to rapid and widespread deployment of software based inference and decision making. There is growing recognition that ML exposes new vulnerabilities in software systems, yet the technical community's understanding of the nature and extent of these vulnerabilities remains limited. We systematize recent findings on ML security and privacy, focusing on attacks identified on these systems and defenses crafted to date. We articulate a comprehensive threat model for ML, and categorize attacks and defenses within an adversarial framework. Key insights resulting from works both in the ML and security communities are identified and the effectiveness of approaches are related to structural elements of ML algorithms and the data used to train them. We conclude by formally exploring the opposing relationship between model accuracy and resilience to adversarial manipulation. Through these explorations, we show that there are (possibly unavoidable) tensions between model complexity, accuracy, and resilience that must be calibrated for the environments in which they will be used.

==> ml-security.tex <==
\section{Security Model}
\label{sec:ml-security}

Before we delve into the specifics of attacks and defenses, we introduce a
comprehensive security model for systems that incorporate a ML component. Our
model characterizes adversaries and risks specific to the presence of a ML model
in a data-processing pipeline. Risks are grouped around three archetypal
security properties: \emph{integrity}, \emph{availability}, and \emph{privacy}.
To structure the space of adversarial capabilities, we propose a threat model
that reflects the two successive phases of ML: \emph{training} and
\emph{inference}. Our work elaborates on previously published threat
models~\cite{barreno2006can,papernot2015limitations} to propose a complete
security model, with insights gained from progress made within the research
community.

\subsection{Adversaries}

Recall the tasks introduced previously while describing 
the data collection process.  First, a supervised \emph{classification} task: assigning malicious or benign
labels to executables. 
Second, an \emph{unsupervised} task: anomaly-based intrusion
detection. Third, a \emph{reinforcement learning} task: a different intrusion
detection model that learns from feedback in the form of system state
indicators. We justify why adversaries would be interested in 
having these systems misbehave (although this is somewhat natural given their
security-centric role). 

When considering the malware classifier, the adversary may
be interested in finding polymorphic variants of malware executables that evade detection,
i.e. are classified as benign by the machine learning model, while retaining
their malware behavior and functionality~\cite{nachenberg1997computer}. If a
machine learning system is used to prevent malicious applications from being
hosted and served on an application marketplace~\cite{enck2009lightweight}, this
attack against the \emph{output integrity} of the machine learning system 
enables the adversary to install malware on smartphones. 

Now, consider the
intrusion detection systems described previously. An adversary with the intent
of penetrating the network will search for variants of attacks not flagged by these
systems~\cite{handley2001network}. The adversary may also compromise the computer network's \emph{availability}. Assume that countermeasures are
taken based on predictions made by the ML model: the adversary can force the
intrusion detection system to produce a specific output that leads to the shutdown
of network infrastructure as a defense maneuver. In such scenarios, the
adversary performs a denial of service.

\subsection{Risks}
As is often the case in security, ML systems face three
types of risks: failure to provide integrity, availability, and privacy.
 Integrity and privacy can both be 
understood at the level of the ML model itself, as well as for the entire 
system deploying machine learning. Availability however primarily makes
sense when considering the system as a whole. We discuss below the range
of adversarial goals that are relate to each risk. 

\boldpara{Integrity} This property is essential in machine learning, and is 
the center of attention for most performance metrics used by machine learning
scientists: e.g., accuracy. However, researchers have shown that the 
integrity of machine learning systems may be compromised by adversaries 
capable of manipulating the inputs of the model~\cite{} or its training 
data~\cite{}. Various risks exist. First, the machine learning model's confidence
may be targeted by an adversary: reducing this value may change the behavior
of the overall system. For instance, an intrusion detection system may 
only raise an alarm when its confidence is over a specified threshold. 
Input misprocessing aims at misleading the model into producing wrong outputs
for some inputs, either modified at the entrance of the pipeline, or at the
input of the model directly. Depending on the task type, the wrong outputs
 differ. For a machine learning classifier, it may classify a legitimate 
 image in the wrong class, or classify noise with confidence. [Add 
 unsupervised/RL] However, 
 when the adversary is capable of subverting the input-output mapping 
 completely, it can control the model and the system's behavior. For instance, 
 it may force an automotive's computer vision system to misprocess a traffic sign, 
 resulting in the car accelerating.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{figs/taxonomy-integrity}
	\caption{\textbf{Integrity axis:}}
	\label{fig:taxonomy-integrity}
\end{figure}

\boldpara{Availability} If the system depends on the output of the machine
learning model to take decisions that impact its availability, it may be
subject to attacks falling under the broad category of denial of service.
For instance, producing vision inputs that force a driverless car to 
stop immediately may cause a denial of service by completely stopping 
traffic on the highway. Machine learning models may also not perform
correctly when some of their input features are corrupted or missing~\cite{}.


\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{figs/taxonomy-availability}
	\caption{\textbf{Availability axis:}}
	\label{fig:taxonomy-availability}
\end{figure}

\boldpara{Privacy and confidentiality} Machine learning models have enough
capacity to capture and memorize elements of their training data~\cite{}. As such, 
it is hard to provide guarantees that participation in a dataset does not
harm the privacy of an individual. Potential risks are adversaries performing
membership test (to know whether an individual is in a dataset or not),
recovering of partially known inputs (use the model to complete an input 
vector with the most likely missing bits), and extraction of the training
data using the model's predictions~\cite{}.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{figs/taxonomy-privacy}
	\caption{\textbf{Privacy and confidentiality axis:}}
	\label{fig:taxonomy-privacy}
\end{figure}


\subsection{Threat Model}
Adversarial Capabilities

Having explicitly described motivations behind
adversarial behaviors against machine learning systems, we now characterize the
attack surface of a model. In Figure~\ref{fig:ml-attack-surface}, we illustrate
a typical machine learning system pipeline and some of the different
representations in which the information is successively transformed. Naturally, adversaries with
varying capability strengths have access to a more or less large portion of the machine learning system's attack surface. Weakest adversaries only have access to the physical
domain upstream of the machine learning system, whereas strong adversaries have
access to the pre-processed representations of the physical domain, or even the
model itself. For instance, in the network intrusion detection scenario, an internal adversary may have access to the model used to distinguish attacks from normal behavior, whereas a weaker eaves-dropping adversary would only have access to TCP dumps of the network traffic. 

\boldpara{Training Phase} During the model's training phase, adversaries
may have access to two types of capabilities:  manipulate the
training data and tamper with the learning algorithm directly. Manipulations
of the training data take various forms, most notably: reading existing data, injection of
additional data,
and modification of existing data~\cite{}. In the case of reinforcement learning,
the adversary may modify the environment in which the agent is evolving as well
as the rewards it is receiving
for instance. One could also envision a scenario
where adversaries tamper with the learning algorithm itself.

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/taxonomy-training}
\caption{\textbf{Training phase axis:}}
\label{fig:taxonomy-training}
\end{figure}

\boldpara{Inference Phase}
Attacks at inference time---\emph{exploratory attacks}~\cite{barreno2006can}---do not tamper with the targeted model but instead either cause it to directly misbehave (integrity) or simply use the attack to collect evidence about the model characteristics (privacy). 

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/taxonomy-inference}
\caption{\textbf{Inference axis:}}
\label{fig:taxonomy-inference}
\end{figure}




